A precise measurement of the $W$-boson mass with the Collider Detector at Fermilab

We present a measurement of the $W$-boson mass, $M_W$, using data corresponding to 2.2/fb of integrated luminosity collected in ppbar collisions at $\sqrt{s}$ = 1.96 TeV with the CDF II detector at the Fermilab Tevatron. The selected sample of 470126 $W\to e\nu$ candidates and 624708 $W\to\mu\nu$ candidates yields the measurement $M_W = 80387\pm 12$ (stat) $\pm 15$ (syst)$ = 80387 \pm 19$ MeV$/c^2$ . This is the most precise single measurement of the $W$-boson mass to date.

==> clc.tex <==
Luminosity is measured using two small-angle Cherenkov luminosity counter 
detectors~\cite{CLC} covering $3.6 <|\eta|<4.6$.  Each detector consists of gas 
Cherenkov counters arranged in 3 concentric layers around the beam pipe.  Signals 
in both detectors that coincide in time with a $p\bar{p}$ bunch crossing are used 
to measure the instantaneous luminosity and to trigger collision events.  Events 
collected with such a trigger, known as ``minimum bias'' events, are used to study 
the detector response to generic inelastic $p\bar{p}$ collisions.  


==> jpsipscale.tex <==
The momentum scale is calibrated using $J/\psi$ decays
by fitting the dimuon mass as a function of mean inverse
$p_T$ of the two muons, and then extrapolating to high 
$p_T$ ($<p_T^{-1}> \approx 0$ GeV$^{-1}$).  The ionizing
material in the tracker is scaled such that the measured
momentum scale is independent of $<p_T^{-1}>$.  This 
procedure results in a calibration accuracy of 0.025\%. 
\par
The $J/\psi$ calibration requires an accurate modelling 
of the muon ionization energy loss in the tracker.  Each 
muon passing through the silicon and COT detectors loses 
on average 9 MeV of energy.  The combined effect on the 
reconstructed $m_{\mu\mu}$ is $\approx 0.6 \% m_{J/\psi}$, 
a factor of $\approx 20$ larger than our total uncertainty.  
Since the ionization energy loss varies only logarithmically
with $p_T$ (Section \ref{sec:ionization}), the relative 
effect on the reconstructed mass is:
\begin{eqnarray}
\begin{array}{lll}
\frac{\Delta m}{m} & = & \frac{\Delta p^{\mu^+}_T}{2 p^{\mu^+}_T} + \frac{\Delta p^{\mu^-}_T}{2 p^{\mu^-}_T}, \\
                   & \approx & \Delta p_T<p_T^{-1}>.
\end{array}
\end{eqnarray}

\noindent
Thus, in a linear fit of $\Delta m/m$ as a function of mean 
inverse $p_T$, a non-zero slope approximately corresponds to 
$\Delta p_T$.  Since we model the ionization energy loss based 
on the known detector material, this slope should be zero.  We 
however find that we need to scale down the ionization energy 
loss from the detector parametrization (Section 
\ref{sec:ionization}) by 6\% to achieve a zero slope.  We show 
the result of this tuning in Fig. \ref{fig:jpsiinvpt}, replacing 
$\Delta m/m$ on the $y-$axis with the relative data momentum 
correction needed to obtain $m_{J/\psi} = 3096.88$ MeV.

\begin{figure}[!tp]
\begin{center}
\epsfysize = 6.cm
\epsffile{psiscale.eps}
\caption{The fractional momentum correction for data as a function 
of the mean inverse momentum of the muons from $J/\psi$ decays.  In 
a linear fit, the intercept corresponds to the scale correction 
relevant for $W$ and $Z$ boson decays, and the slope corresponds to 
the remaining unmodelled ionization energy loss after material tuning. 
The uncertainties are statistical only.}
\label{fig:jpsiinvpt}
\end{center}
\end{figure}

Each $\Delta p/p$ value in Fig. \ref{fig:jpsiinvpt} is extracted 
via a binned likelihood fit to the $m_{\mu\mu}$ distribution for 
each $<p_T^{-1}>$ range.  Since the mass resolution varies significantly
with $<p_T^{-1}>$, the fit ranges are adjusted from $3.08 \pm 0.13$ GeV 
for $<p_T^{-1}> = (0.1,0.15)$ to $3.08 \pm 0.08$ GeV for 
$<p_T^{-1}> = (0.45,0.5)$.  Background is modelled as a linear function
of $m_{\mu\mu}$, with parameters determined from a region outside the mass 
fit window with an equal size to that used in the mass fit.  The result of 
the fit in the $<p_T^{-1}> = (0.15,0.2)$ range is shown in Fig. 
\ref{fig:jpsimassfit}.  

\begin{figure}[!tp]
\begin{center}
\epsfysize = 6.cm
\epsffile{psimassbin2.eps}
\caption{The $m_{\mu\mu}$ fit to data (points) with $<p_T^{-1}> = (0.15,0.2)$.  
The best fit to the $m_{\mu\mu} = 3.08 \pm 0.12$ region corresponds to a 
momentum scale correction of $(-1.54 \pm 0.09) \times 10^{-3}$.  The 
uncertainty is statistical only.}
\label{fig:jpsimassfit}
\end{center}
\end{figure}

Systematic uncertainties on the momentum scale correction extracted from
$J/\psi \rightarrow \mu\mu$ decays result from (Table \ref{tbl:psiupssys}):  
incompleteness of the QED and energy loss models; longitudinal variations 
of the magnetic field; the statistical limit of the ionizing material 
correction; statistical limits on the tracker alignment corrections; 
sensitivity of the result to the fit region definition; potential 
momentum-dependent trigger inefficiency; choice of background parametrization; 
tracker hit resolution modelling; and uncertainty on the world-average 
$J/\psi$ mass.
\par
At low muon $p_T$ (high $<p_T^{-1}>$), the mass fits become more sensitive to 
QED and energy loss modelling because of the better mass resolution and higher 
statistics.  Since we only model the mean ionization energy loss, our modelling 
of the mass region below the peak is imperfect.  Additionally, neglecting 
higher-order QED corrections affects our modelling of this region.  We study 
possible bias from our incomplete model by changing the $m_{J/\psi}$ value in 
the photon radation probability function such that the $\chi^2$ of the inclusive 
$m_{\mu\mu}$ fit is minimized.  We find that this change affects $\Delta p/p$ 
by $0.2 \times 10^{-3}$.
\par
If there is a relative tilt between the solenoid and the tracker, the extracted 
momentum scale correction will have a linear $\cot\theta$ dependence.  In addition,
incomplete corrections of the magnetic field nonuniformities near the ends of the 
solenoid can cause a quadratic $\cot\theta$ variation.  We use $J/\psi$ muon decays 
with $|\Delta\cot\theta (\mu\mu)| < 0.1$ to study the extracted $\Delta p/p$ as a 
function of $\cot\theta$.  We find that if we correct for the observed quadratic
dependence, the extracted $\Delta p/p$ changes by $0.1 \times 10^{-3}$.
\par
In the linear fit in Fig. \ref{fig:jpsiinvpt}, the uncertainty on the scale correction
is dominated by the uncertainty on the ionization energy loss.  Fixing the energy 
loss to zero results in a scale correction uncertainty of $0.01 \times 10^{-3}$.  We 
thus take the uncertainty due to the material correction to be that obtained in the 
linear fit, $0.06 \times 10^{-3}$.
\par
The statistical uncertainties on the $J/\psi$ alignment corrections (equations 
\ref{eq:jpsicurvcor} and \ref{eq:zscale}) have a $0.05 \times 10^{-3}$ effect on 
$\Delta p/p$.  We test our model of the $m_{\mu\mu}$ lineshape by changing the 
fit range by $\pm 20\%$, and find a $\pm 0.05 \times 10^{-3}$ change in 
$\Delta p/p$.
\par
We apply the same $p_T$ thresholds offline as in the trigger for muons with CMU 
segments.  Since we do not model a $p_T$-dependent trigger efficiency, any 
inefficiency could cause a bias in the reconstructed $m_{\mu\mu}$ mass.  We 
investigate this possibility by varying the offline $p_T$ thresholds by $\pm 5\%$, 
and find a $\Delta p/p$ variation of $\pm 0.04 \times 10^{-3}$.
\par
The quality of the fit is highly sensitive to the hit resolution model, but the 
momentum scale correction is not.  Changing the simulated COT hit resolution by 
$\pm 10 \mu$m, which corresponds to $> 10\sigma$, results in a 
$\pm 0.03 \times 10^{-3}$ change in $\Delta p/p$.  We include this in our systematic 
uncertainty estimate.  
\par
A $\pm 0.03 \times 10^{-3}$ uncertainty on $\Delta p/p$ from the background model 
is determined by changing its linear dependence on $m_{\mu\mu}$ to a constant.  
Finally, the world-average $J/\psi$ mass value used in this measurement contributes 
$\pm 0.01 \times 10^{-3}$ to the uncertainty on $\Delta p/p$.

\begin{table*}[htbp]
\begin{center}
\begin{tabular}{lccc}
\hline
\hline
Source                         &  $J/\psi$ ($\times 10^{-3}$) &  $\Upsilon$ ($\times 10^{-3}$)  & Common ($\times 10^{-3}$) \\
\hline
QED and energy loss model      & 0.20   &  0.13  &  0.13  \\
Magnetic field nonuniformities & 0.10   &  0.12  &  0.10  \\
Beam constraint bias	       & N/A    &  0.06  &  0     \\
Ionizing material scale        & 0.06   &  0.03  &  0.03  \\
COT alignment corrections      & 0.05   &  0.03  &  0.03  \\
Fit range	               & 0.05   &  0.02  &  0.02  \\
$p_T$ threshold		       & 0.04   &  0.02  &  0.02  \\
Resolution model	       & 0.03   &  0.03  &  0.03  \\
Background model               & 0.03   &  0.02  &  0.02  \\
World-average mass value       & 0.01   &  0.03  &  0     \\
\hline
Statistical                    & 0.01   &  0.06  &  0     \\
\hline
Total                          & 0.25   & 0.21   &  0.17  \\
\hline
\hline
\end{tabular}
\caption{Uncertainties on the momentum scale correction derived from the 
$J/\psi$ and $\Upsilon$ mass measurements. }
\label{tbl:psiupssys}
\end{center}
\end{table*}


==> lpm.tex <==
The Bethe-Heitler bremsstrahlung spectrum is modified by screening effects at high $y$ (where $y = E_\gamma / E_e$ and $0 < y < 1$) and by the Landau-Pomeranchuk-Migdal (LPM) suppression 
 for $y \sim 0.001$. We also model the dielectric suppression of bremsstrahlung for $y \sim 10^{-5}$, but its effect on the $W$ boson mass measurement is $< 1$ MeV and therefore negligible. We generate and propagate bremsstrahlung photons for $y > 10^{-4}$. Lowering this cutoff has $< 1$ MeV
 impact on the analysis, since the softer photons are already suppressed.  
 The LPM suppression of bremsstrahlung is caused by multiple scattering which
 interferes with the formation of the photon. As $y$ decreases, the photon formation length increases and multiple scattering is more likely to suppress the photon emission. Denser materials with shorter
 radiation lengths therefore cause more LPM suppression. 

We have also studied the modification of the bremsstrahlung spectrum according to EEDL~\cite{riddick}, which reduces the bremstrahlung rate above $y \sim 0.3$ by $\approx 1$\%
 compared to the spectrum we use. Retuning all of our key parameters with the EEDL spectrum, we find that our passive material model has to be retuned by 0.5\%, with a corresponding
 change in the energy scale by 5 MeV~\cite{riddick}. Since the EEDL correction is complicated and not strongly motivated, and the effect on our measurement is small, we do not use
 it as our default model. 
  
The spectrum we use here is the same as in~\cite{dukeSim, prd} including the LPM and dielectric suppression, but the modelling of the LPM suppression  has been improved. In the following section, we describe
 the improvement in the modeling of the LPM effect. 

The description of the calorimeter has also been significantly improved compared to~\cite{dukeSim, prd}, based on detailed studies using GEANT4~\cite{geantElectron,
 geantPhoton, geantNonLin}.

 In our previous analysis~\cite{prd}, we had calculated the LPM suppression under the assumption that the bremsstrahlung occurred in silicon. In the
 current analysis, we use different materials in different regions of the tracking volume, depending on how the detectors were built. 

 We have studied the documentation~\cite{materialEstimates}
  on the silicon detector construction to understand the material composition of the various components. In some regions the 
 material composition is very simple; beryllium for the beampipe and the SVX bulkheads, silicon for the sensors and carbon for the COT inner wall. For these regions we calculate the LPM suppression corresponding to these
 respective materials directly. A significant number of  radiation lengths are also found
 in the SVX port card region and the L00/SVX/ISL hybrids. These regions contain mixtures of various materials. The hybrids contain light materials such as
 beryllium oxide, aluminum nitride and glass, and heavy materials such as lead, barium, titanium, copper, 
 lead/tin (solder), silver and gold. The portcards contain the same heavy metals, and lighter materials like alumina, hydrocarbons and glass. The
 region of the portcards also contains a lot of the cabling, which is a combination of kapton and copper. All of this information is encoded
 in the GEANT description of the detector in CDFSim. 

 We have experimentally constrained the total amount of ionization energy loss (from the fits to the $J/\psi \rightarrow \mu \mu$ and $\Upsilon
 \rightarrow \mu \mu$ masses~\cite{momentumScale}), 
 and the total amount of radiation lengths (from the tail of the $E/p$ distribution as discussed below). 
 Silimap uses all the details encoded in CDFSim to compute the  total ionization energy loss and total radiation lengths in each 3D $(r, \phi, z)$ 
 bin with fine spatial granularity. Silimap does not provide the details of the material composition, therefore we encode the dominant materials
 used in the detector construction directly into DukeSim, based on the information in~\cite{materialEstimates} for their respective fractions in
 each detector region. Furthermore, we apply the constraints that in each 3D spatial bin, the total ionization energy loss and the total radiation
 lengths calculated by the DukeSim code coincides with the respective values from CDFSim (as stored in Silimap). 
 
 Given these two constraints from GEANT/CDFSim, the relevant parameter to describe any material is the ionization energy loss per radiation length 
 of the material. Considering the various materials found in the detector:  beryllium loses 105 MeV/$X_0$, while lead and 
 gold are at the other end of this parameter's range with 7 MeV/$X_0$. Relatively  
 light materials like beryllium oxide, carbon and kapton lose about 75 MeV/$X_0$, while silicon, aluminum, glass, silica, alumina, and
 aluminum nitride lose about 40 MeV/$X_0$. Copper and tin lose about 17 MeV/$ X_0$. Almost all of the materials used in the tracker construction
 fall into these five categories, with materials in the same category 
 having similar MeV/$X_0$ values and similar LPM suppression within 10\%. Metals like barium and silver are well-approximated by a mixture of copper and
 gold. 

 In the hybrids, we use the information in~\cite{materialEstimates} to 
 describe the light material by a mixture of 50\% beryllium oxide and 50\% glass, and 
 the heavy component is described by gold to represent all the heavy metals. 
 In each 3D spatial bin, the amount of light and heavy materials is constrained by 
 the values of the total ionization energy loss and total radiation length  given by Silimap. 
 Similarly  in the portcard region, the dominant heavy material is copper due to the cables, but the portcards contribute denser
 metal (represented by gold) for a relative fraction of 19\% of the radiation lengths. The light material in the portcard region is 63\% kapton 
 due to the cables, with 37\% beryllium oxide. Finally, in the COT active volume, the light 
 materials are the gas and kapton field sheets, and the heavy metals (eg. the wires) contribute steel and tungsten/gold in the relative fractions of 65\% and 35\%
 respectively. 

In summary, we use  different pairs of light/heavy materials for 
 the different regions; (50\% beryllium oxide + 50\% glass)/gold in all the regions of the hybrids, 
 (37\% beryllium oxide + 63\% kapton)/(19\% gold + 81\% copper) in the portcard region and kapton/(35\% gold + 65\% copper) in the COT active volume. 


 The uncertainty in the energy scale is due to the copper to gold ratio estimated
  in the portcard  region, and the beryllium oxide to glass ratio
 estimated in the hybrids. If we vary the gold fraction in the portcard region
 from zero to 40\%, we find that the fitted energy scale changes by 8 MeV. This corresponds to a relative variation of 100\% of the amount of very heavy 
 metals in the portcard region. Similarly, if we vary the beryllium oxide to glass proportion
  from zero to 100\% in the hybrids, we find the fitted energy scale changes by 7 MeV. This corresponds to a relative variation of 100\% of the glass fraction in
 the hybrids. 

 Conservatively, 
 we add the energy scale variations linearly since the errors in the material estimates might be correlated. 
 The material accounting in~\cite{materialEstimates} is meant to be accurate
 to 10\% of itself, and our categorization of the materials into the five groups is also representative of their properties within 10\%. 
 Again to be conservative, we add these modeling errors linearly to allow for correlation. Thus, we
  take 20\% of the 15 MeV variation as the uncertainty due to mis-modeling of the LPM suppression in 
 DukeSim, amounting to a 3 MeV uncertainty on the energy scale. 

 The $y$-dependence of the LPM suppression has been computed~\cite{spencerKlein} and measured~\cite{plAnthony, plAnthonyPRD}.
  We use the calculated parameterization
 and apply additional tuning based on the calculation-to-data comparisons in~\cite{riddick} and~\cite{plAnthony, plAnthonyPRD}.
  Given the high precision of the LPM measurements,  
 the uncertainty due to the $y$-dependent shape of the LPM parameterization is negligible. 
 

